A Framework for Extending microKanren with Constraints

We present a framework for building CLP languages with symbolic constraints based on microKanren, a domain-specific logic language shallowly embedded in Racket. We rely on Racket's macro system to generate a constraint solver and other components of the microKanren embedding. The framework itself and the constraints' implementations amounts to just over 100 lines of code. Our framework is both a teachable implementation for CLP as well as a test-bed and prototyping tool for symbolic constraint systems.

==> eptcsdata.tex <==
\providecommand{\firstpage}{135}
\providecommand{\publicationstatus}{S. Schwarz and J. Voigtl\"ander (Eds.): 29th and 30th Workshops\\
on (Constraint) Logic Programming and 24th International\\
Workshop on Functional and (Constraint) Logic Programming\\
(WLP'15/'16/WFLP'16).\\
EPTCS 234, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.234.10}{10.4204/EPTCS.234.10}}

